How well can we guess theoretical uncertainties?

The problem of estimating the effect of missing higher orders in perturbation theory is analyzed with emphasis in the application to Higgs production in gluon-gluon fusion. Well-known mathematical methods for an approximated completion of the perturbative series are applied with the goal to not truncate the series, but complete it in a well-defined way, so as to increase the accuracy - if not the precision - of theoretical predictions. The uncertainty arising from the use of the completion procedure is discussed and a recipe for constructing a corresponding probability distribution function is proposed.

==> defs.tex <==
%---
%\usepackage{colordvi}
%\usepackage{epsfig}
%\usepackage{axodraw}
%\usepackage{epsfig}
\usepackage{graphicx}
%\usepackage{rotate}
%\usepackage{latexsym}
\usepackage{amssymb}
%\usepackage[reqno,tbtags]{amsmath}
%\usepackage{multirow}
\RequirePackage{mathptmx}
\RequirePackage[T1]{fontenc}
%---
\usepackage{heppennames2}
\usepackage{lhchiggs}
\usepackage{cernunits}

%\usepackage{lineno}
\usepackage{color}
\newcommand{\CheckMe}[1]{{\color{red}\bfseries $\blacktriangleright$ {#1} $\blacktriangleleft$}\xspace}
\newcommand{\CheckG}[1]{{\color{blue}\bfseries $\blacktriangleright$ {#1} $\blacktriangleleft$}\xspace}
\usepackage{url} 

%---
\DeclareSymbolFont{forjmath}{OT1}{cmr}{m}{sl}
\DeclareMathSymbol{\Jmath}{\mathord}{forjmath}{'021}
\def\jmath{\Jmath}
\DeclareFontFamily{OT1}{cmr}{}
\DeclareFontFamily{OT1}{cmss}{}
%--
\hyphenation{ma-ni-pu-la-tions}
%\allowdisplaybreaks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% basic data for the eprint:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\textwidth=6.5in  \textheight=8.7in
\leftmargin=-0.8in   \topmargin=-0.20in
\hoffset=-.85in

%% preprint number data:
%% Change the preprint number below to your institutional preprint number
\newcommand\pubdate{\today}
%% If you will submit to hep-ex, change hep-ph to hep-ex below
%% Do not change yymmnnn; this will be automatically converted
%% to the Los Alamos hep number during the submission process
\newcommand\hepnumber{hep-ph/yymmnnn}

%%  address and funding acknowledgment data:
\def\csumb{Dipartimento di Fisica Teorica, Universit\`a di Torino, Italy\\
           INFN, Sezione di Torino, Italy}
\def\support{\footnote{Work supported by MIUR under contract
    2001023713$\_$006 and by Compagnia di San Paolo under contract ORTO11TPXK.}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   document style macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Title#1{\begin{center} {\Large\bf #1 } \end{center}}
\newcommand{\Authors}[2]{\begin{center}{ \sc #1 \hspace{0.1cm} {\rm and}
\hspace{0.1cm} #2} \end{center}}
\def\Author#1{\begin{center}{ \sc #1} \end{center}}
\def\Address#1{\begin{center}{ 
%\normalsize \bfseries \it #1} \end{center}}
\normalsize \bfseries \itshape #1} \end{center}}
\def\andauth{\begin{center}{and} \end{center}}
\def\submit#1{\begin{center}Submitted to {\sl #1} \end{center}}
\newcommand\pubblock{\rightline{\begin{tabular}{l} \\
         \pubdate\\  \end{tabular}}}
\newenvironment{Abstract}{\begin{quotation}  }{\end{quotation}}
\newenvironment{Presented}{\begin{quotation} \begin{center}
             Presented at the\end{center}
      \begin{center}\begin{large}}{\end{large}\end{center} \end{quotation}}
\def\Acknowledgments{\bigskip  \bigskip \begin{center}
          \large\bf Acknowledgments\end{center}}
\def\email#1{\footnote{\tt EMAIL: #1}}
\makeatletter
%\def\section{\@startsection{section}{0}{\z@}{5.5ex plus .5ex minus
% 1.5ex}{2.3ex plus .2ex}{\large\bf}}
%\def\subsection{\@startsection{subsection}{1}{\z@}{3.5ex plus .5ex minus
% 1.5ex}{1.3ex plus .2ex}{\normalsize\bf}}
%\def\subsubsection{\@startsection{subsubsection}{2}{\z@}{-3.5ex plus
%-1ex minus  -.2ex}{2.3ex plus .2ex}{\normalsize\sl}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% small size table and figure captions %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\@makecaption}[2]{%
   \vskip 10pt
   \setbox\@tempboxa\hbox{\small #1: #2}
   \ifdim \wd\@tempboxa >\hsize     % IF longer than one line:
       \small #1: #2\par          %   THEN set as  ordinary paragraph.
     \else                        %   ELSE  center.
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}
   \fi}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros to collapse citation numbers to ranges %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \citenum emits the plain citation number without ornament
% \citea puts it's argument into the ornamentation for citations
% thus \cite{foo} is equivalent to \citea{\citenum{foo}}
 \def\citenum#1{{\def\@cite##1##2{##1}\cite{#1}}}
\def\citea#1{\@cite{#1}{}}
%
% Collapse citation numbers to ranges.  Non-numeric and undefined labels
% are handled.  No sorting is done.  E.g., 1,3,2,3,4,5,foo,1,2,3,,4,5
% gives 1,3,2-5,foo,1-3,,4,5
\newcount\@tempcntc
\def\@citex[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \@tempcnta\z@\@tempcntb\m@ne\def\@citea{}\@cite{\@for\@citeb:=#2\do
    {\@ifundefined
       {b@\@citeb}{\@citeo\@tempcntb\m@ne\@citea\def\@citea{,}{\bf }\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
    {\setbox\z@\hbox{\global\@tempcntc0\csname b@\@citeb\endcsname\relax}%
     \ifnum\@tempcntc=\z@ \@citeo\@tempcntb\m@ne
       \@citea\def\@citea{,}\hbox{\csname b@\@citeb\endcsname}%
     \else
      \advance\@tempcntb\@ne
      \ifnum\@tempcntb=\@tempcntc
      \else\advance\@tempcntb\m@ne\@citeo
      \@tempcnta\@tempcntc\@tempcntb\@tempcntc\fi\fi}}\@citeo}{#1}}
\def\@citeo{\ifnum\@tempcnta>\@tempcntb\else\@citea\def\@citea{,}%
  \ifnum\@tempcnta=\@tempcntb\the\@tempcnta\else
  {\advance\@tempcnta\@ne\ifnum\@tempcnta=\@tempcntb \else\def\@citea{--}\fi
    \advance\@tempcnta\m@ne\the\@tempcnta\@citea\the\@tempcntb}\fi\fi}
%
\newcommand\KW[1]{\vskip .5pt \vbox{\small Keywords:\ #1}}
\newcommand\PACS[1]{\vskip .5pt \vbox{\small PACS:\ #1}}
\newcommand\secstyle{\bfseries\raggedright}
\renewcommand\section{\@startsection{section}{1}{\z@}%
                                   {3.5ex \@plus 1.3ex \@minus .7ex}%
                                   {2.3ex \@plus.4ex \@minus .4ex}%
                                   {\normalfont\large\secstyle}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {2.3ex\@plus 1ex \@minus .5ex}%
                                   {1.2ex \@plus .3ex \@minus .3ex}%
                                   {\normalfont\normalsize\secstyle}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                   {2.3ex\@plus 1ex \@minus .5ex}%
                                   {1ex \@plus .2ex \@minus .2ex}%
                                   {\normalfont\normalsize\secstyle}}% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% corrects bad spacing in LaTeX multiple line equations
% replace eqnarray with Eanarray (or use abbreviations
% in econfmacros2.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newenvironment{Eqnarray}%
%   {\arraycolsep 0.14em\begin{eqnarray}}{\end{eqnarray}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  personal abbreviations and macros
%    the following package contains macros used in this document:
%--
%- Local macros
%--
\DeclareRobustCommand{\PA}{\HepParticle{A}{}{}\Xspace}
\DeclareRobustCommand{\PU}{\HepParticle{U}{}{}\Xspace}
\DeclareRobustCommand{\PV}{\HepParticle{V}{}{}\Xspace}
\DeclareRobustCommand{\PS}{\HepParticle{S}{}{}\Xspace}
\DeclareRobustCommand{\PT}{\HepParticle{T}{}{}\Xspace}
\DeclareRobustCommand{\PX}{\HepParticle{X}{}{}\Xspace}
\DeclareRobustCommand{\PY}{\HepParticle{Y}{}{}\Xspace}
\DeclareRobustCommand{\Pf}{\HepParticle{f}{}{}\Xspace}
\DeclareRobustCommand{\PAf}{\HepAntiParticle{\Pf}{}{}\Xspace}
\DeclareRobustCommand{\PF}{\HepParticle{F}{}{}\Xspace}
\DeclareRobustCommand{\PI}{\HepParticle{I}{}{}\Xspace}
\DeclareRobustCommand{\PM}{\HepParticle{M}{}{}\Xspace}
\DeclareRobustCommand{\Ph}{\HepParticle{h}{}{}\Xspace}
\DeclareRobustCommand{\Phad}{\HepParticle{h}{}{}\Xspace}
\newcommand{\FR}{\rm{\scriptscriptstyle{FR}}}
\newcommand{\AC}{\rm{\scriptscriptstyle{AC}}}
\newcommand{\myLO}{\rm{\scriptscriptstyle{LO}}}
\newcommand{\myNLO}{\rm{\scriptscriptstyle{NLO}}}
\newcommand{\myYM}{\rm{\scriptscriptstyle{YM}}}
%\newcommand{\myGF}{\rm{\scriptscriptstyle{GF}}}
\newcommand{\myFP}{\rm{\scriptscriptstyle{FP}}}
\newcommand{\OS}{\mathrm{OS}}
\newcommand{\CPP}{\mathrm{CPP}}
\newcommand{\mUV}{\mathrm{UV}}
\newcommand{\mBW}{\mathrm{BW}}
\newcommand{\OFS}{\mathrm{OFS}}
\newcommand{\Lint}{\mathrm{int}}
\newcommand{\mySM}{\rm{\scriptscriptstyle{SM}}}
\newcommand{\MSSM}{\rm{\scriptscriptstyle{MSSM}}}
\newcommand{\BSM}{\rm{\scriptscriptstyle{BSM}}}
\newcommand{\myEW}{{\scriptscriptstyle{E}\scriptscriptstyle{W}}}
\newcommand{\ssA}{{\mathrm{A}}}
\newcommand{\ssB}{{\mathrm{B}}}
\newcommand{\ssC}{{\mathrm{C}}}
\newcommand{\ssQ}{{\mathrm{Q}}}
\newcommand{\ssF}{{\mathrm{F}}}
\newcommand{\ssR}{{\mathrm{R}}}
\newcommand{\ssD}{{\mathrm{D}}}
\newcommand{\ssU}{{\mathrm{U}}}
\newcommand{\ssL}{{\mathrm{L}}}
\newcommand{\ssY}{{\mathrm{Y}}}
\newcommand{\ssP}{{\mathrm{P}}}
\newcommand{\ssS}{{\mathrm{S}}}
\newcommand{\ssH}{{\mathrm{H}}}
\newcommand{\ssV}{{\mathrm{V}}}
\newcommand{\ssM}{{\mathrm{M}}}
\newcommand{\ssN}{{\mathrm{N}}}
\newcommand{\ssK}{{\mathrm{K}}}
\newcommand{\ssG}{{\mathrm{G}}}
\newcommand{\sH}{\mathrm{H}}
\newcommand{\HH}{\mathrm{HH}}
\newcommand{\VV}{\mathrm{VV}}
\newcommand{\ssh}{{\mathrm{h}}}
\newcommand{\ssW}{{\mathrm{W}}}
\newcommand{\ssWW}{{\scriptscriptstyle{WW}}}
\newcommand{\ssT}{{\mathrm{T}}}
\newcommand{\ssZ}{{\mathrm{Z}}}
\newcommand{\bqas}{\begin{eqnarray*}}
\newcommand{\eqas}{\end{eqnarray*}}
\newcommand{\nl}{\nonumber\\}
\def\mnew{\mpar{\hfil NEW \hfil}\ignorespaces}
\newcommand{\lpar}{\left(}                            % bracketing
\newcommand{\rpar}{\right)} 
\newcommand{\lrbr}{\left[}
\newcommand{\rrbr}{\right]}
\newcommand{\lcbr}{\left\{}
\newcommand{\rcbr}{\right\}} 
\newcommand{\rbrak}[1]{\lrbr#1\rrbr}
\newcommand{\bq}{\begin{equation}}                    % equationing
\newcommand{\eq}{\end{equation}}
\newcommand{\bqa}{\arraycolsep 0.14em\begin{eqnarray}}
\newcommand{\eqa}{\end{eqnarray}}
\newcommand{\ba}[1]{\begin{array}{#1}}
\newcommand{\ea}{\end{array}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bei}{\begin{itemize}}
\newcommand{\eei}{\end{itemize}}
\newcommand{\eqn}[1]{Eq.(\ref{#1})}
\newcommand{\eqns}[2]{Eqs.(\ref{#1})--(\ref{#2})}
\newcommand{\eqnss}[1]{Eqs.(\ref{#1})}
\newcommand{\eqnsc}[2]{Eqs.(\ref{#1}) and (\ref{#2})}
\newcommand{\eqnst}[3]{Eqs.(\ref{#1}), (\ref{#2}) and (\ref{#3})}
\newcommand{\eqnsf}[4]{Eqs.(\ref{#1}), (\ref{#2}), (\ref{#3}) and (\ref{#4})}
\newcommand{\eqnsv}[5]{Eqs.(\ref{#1}), (\ref{#2}), (\ref{#3}), (\ref{#4}) and (\ref{#5})}
\newcommand{\tbn}[1]{Tab.~\ref{#1}}
\newcommand{\tabn}[1]{Tab.~\ref{#1}}
\newcommand{\tbns}[2]{Tabs.~\ref{#1}--\ref{#2}}
\newcommand{\tabns}[2]{Tabs.~\ref{#1}--\ref{#2}}
\newcommand{\tbnsc}[2]{Tabs.~\ref{#1} and \ref{#2}}
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\figs}[2]{Figs.~\ref{#1}--\ref{#2}}
\newcommand{\sect}[1]{Section~\ref{#1}}
\newcommand{\sects}[2]{Section~\ref{#1} and \ref{#2}}
\newcommand{\sectm}[2]{Section~\ref{#1} -- \ref{#2}}
\newcommand{\subsect}[1]{Subsection~\ref{#1}}
\newcommand{\subsectm}[2]{Subsection~\ref{#1} -- \ref{#2}}
\newcommand{\appendx}[1]{Appendix~\ref{#1}}
\newcommand{\hsp}{\hspace{.5mm}}
\def\negs{\hspace{-0.26in}}
\def\negsh{\hspace{-0.13in}}
%--
\newcommand{\hatp}{{\hat p}}
\newcommand{\barq}{\overline q}
\newcommand{\barb}{\overline b}
\newcommand{\bmid}{\Bigr|}
\newcommand{\intrp}{\int_0^{\infty}}
\newcommand{\intMB}{\int_{-i\,\infty}^{+i\,\infty}}
\newcommand{\ord}[1]{{\cal O}\lpar#1\rpar}
\newcommand{\oD}{{\overline \Delta}}
%--
\newcommand{\Mbp}{\mathswitch {m_{\PQbpr}}}
\newcommand{\Mtp}{\mathswitch {m_{\PQtpr}}}
\newcommand{\Mlp}{\mathswitch {m_{\Pl'}}}
\newcommand{\Mnp}{\mathswitch {m_{\PGnl'}}}
\newcommand{\Bref}[1]{Ref.~\cite{#1}}
\newcommand{\Brefs}[1]{Refs.~\cite{#1}}
\newcommand{\Fref}[1]{Fig.~[#1]}
%--
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\etal}{\emph{et al.}}
%\newcommand{\cf}{\emph{cf.\xspace}}
%\newcommand{\SPp}{~}       %% space before punctuation in math
%--
%\newcommand{\mv}{\mathswitch {M_{\ssV}}}
\newcommand{\mv}{\mathswitch {M_{\PV}}}
\newcommand{\mh}{\mathswitch {M_{\PH}}}
\newcommand{\mw}{\mathswitch {M_{\PW}}}
\newcommand{\mbw}{\mathswitch {m_{\PW}}}
\newcommand{\mbws}{\mathswitch {m^2_{\PW}}}
\newcommand{\mz}{\mathswitch {M_{\PZ}}}
\newcommand{\mhs}{\mathswitch {M^2_{\PH}}}
\newcommand{\mPs}{\mathswitch {M^2_{\PS}}}
\newcommand{\mBh}{\mathswitch {{\overline M}_{\PH}}}
\newcommand{\mBhs}{\mathswitch {{\overline M}^2_{\PH}}}
\newcommand{\mhq}{\mathswitch {M^4_{\PH}}}
\newcommand{\mws}{\mathswitch {M^2_{\PW}}}
\newcommand{\mzs}{\mathswitch {M^2_{\PZ}}}
\newcommand{\mt}{\mathswitch {M_{\PQt}}}
\newcommand{\mb}{\mathswitch {M_{\PQb}}}
\newcommand{\mts}{\mathswitch {M^2_{\PQt}}}
\newcommand{\mbs}{\mathswitch {M^2_{\PQb}}}
\newcommand{\cph}{\mathswitch {s_{\PH}}}
\newcommand{\cpw}{\mathswitch {s_{\PW}}}
\newcommand{\cpwz}{\mathswitch {s_{\PW}, s_{\PZ}}}
\newcommand{\cpz}{\mathswitch {s_{\PZ}}}
\newcommand{\cpt}{\mathswitch {s_{\PQt}}}
\newcommand{\muh}{\mathswitch {\mu_{\PH}}}
\newcommand{\muhs}{\mathswitch {\mu^2_{\PH}}}
\newcommand{\gh}{\mathswitch {\gamma_{\PH}}}
\newcommand{\GOS}{\mathswitch {\Gamma_{\OS}}}
\newcommand{\GOL}{\mathswitch {\overline\Gamma}}
\newcommand{\muol}{\mathswitch {\overline\mu}}
\newcommand{\GOSu}{\mathswitch {\Gamma^{\OS}}}
\newcommand{\shat}{\mathswitch {\hat s}}
\newcommand{\muR}{\mathswitch {\mu_{\ssR}}}
\newcommand{\muF}{\mathswitch {\mu_{\ssF}}}
\newcommand{\muRs}{\mathswitch {\mu^2_{\ssR}}}
\newcommand{\muFs}{\mathswitch {\mu^2_{\ssF}}}
\newcommand{\tot}{{\mbox{\scriptsize tot}}}
\newcommand{\myprod}{{\mbox{\scriptsize prod}}}
\newcommand{\prop}{{\mbox{\scriptsize prop}}}
\newcommand{\dec}{{\mbox{\scriptsize dec}}}
\newcommand{\ndec}{{\mbox{\scriptsize non-dec}}}
%\newcommand{\int}{{\mbox{\scriptsize int}}}
\newcommand{\kcut}{{\mbox{\scriptsize cut}}}
\newcommand{\ch}{{\mbox{\scriptsize ch}}}
\newcommand{\inv}{{\mbox{\scriptsize inv}}}
\newcommand{\bos}{{\mbox{\scriptsize bos}}}
\newcommand{\peak}{{\mbox{\scriptsize peak}}}
\newcommand{\ren}{{\mbox{\scriptsize ren}}}
\newcommand{\mdiv}{{\mbox{\scriptsize div}}}
\newcommand{\eff}{{\mbox{\scriptsize eff}}}
\newcommand{\DR}{{\mbox{\scriptsize DR}}}
\newcommand{\full}{{\mbox{\scriptsize full}}}
\newcommand{\bin}{{\mbox{\scriptsize in}}}
\newcommand{\bout}{{\mbox{\scriptsize out}}}
\newcommand{\ac}{{\mbox{\scriptsize all}}}
\newcommand{\esp}{{\mbox{\scriptsize exp}}}
\newcommand{\trac}{{\mathrm{Tr}}}
\newcommand{\gfix}{{\mbox{\scriptsize gf}}}
\newcommand{\fact}{{\mbox{\scriptsize fc}}}
\newcommand{\nfact}{{\mbox{\scriptsize nfc}}}
\newcommand{\spin}{{\mbox{\scriptsize spin}}}
\newcommand{\fer}{{\mbox{\scriptsize fer}}}
\newcommand{\HO}{{\mathrm{HO}}}
\newcommand{\FP}{{\mathrm{FP}}}
\newcommand{\intfxy}[2]{\int_{\scriptstyle 0}^{\scriptstyle 1}\,d#1\,
                        \int_{\scriptstyle 0}^{\scriptstyle #1}\,d#2}
\newcommand{\li}[2]{\mathrm{Li}_{#1}\lpar\displaystyle{#2}\rpar} % polylog
%--
\newcommand{\eG}[1]{\mathswitch \Gamma\lpar #1 \rpar}
\newcommand{\eGs}[1]{\mathswitch \Gamma^2\lpar #1 \rpar}
\newcommand{\ep}{\mathswitch \varepsilon}
\newcommand{\epb}{\mathswitch {\overline\varepsilon}}
\newcommand{\spro}[2]{{#1}\cdot{#2}}
\newcommand{\sspro}[2]{{p_{#1}}\cdot{p_{#2}}}
\providecommand\HTO{{\sc HTO}}
\providecommand\POWHEG{{\sc POWHEG}}
\providecommand\iHixs{{\sc iHixs}}
%--
\newcommand{\stw}{s_{\theta}}             % bare, Lagrangian parameters
\newcommand{\ctw}{c_{\theta}}
\newcommand{\stws}{s_{\theta}^2}
\newcommand{\ctws}{c_{\theta}^2}
%
\newcommand\mybar[1]{\ensuremath{\bar{#1}}}
\newcommand\mytil[1]{\ensuremath{\tilde{#1}}}
%
%\newcommand{\OM}{{\mybar{M}}}
%\newcommand{\OMs}{{\mybar{M}}^2}
%\newcommand{\OMzs}{{\mybar{M}}^2_0}
%\newcommand{\OMzq}{{\mybar{M}}^4_0}
%\newcommand{\OMH}{{\mybar{M}}_{\PH}}
%\newcommand{\OMHs}{{\mybar{M}}^2_{\PH}}
%\newcommand{\OMHq}{{\mybar{M}}^4_{\PH}}
\newcommand{\cth}{{\hat c}_{\theta}}
\newcommand{\sth}{{\hat s}_{\theta}}
\newcommand{\cths}{{\hat c}^2_{\theta}}
\newcommand{\sths}{{\hat s}^2_{\theta}}
\newcommand{\sthq}{{\hat s}^4_{\theta}}
%\newcommand{\PZB}{{\mybar{\PZ}}}
%\newcommand{\myPAB}{{\mybar{\PA}}}
%\newcommand{\HB}{{\mybar{\PH}}}
%\newcommand{\phib}{{\mybar{\upphi}}}
\newcommand{\HSs}{{\Lambda^2}}
%
\DeclareRobustCommand{\PWpmmu}{\HepParticle{\PW}{\mu}{\pm}\Xspace}
\DeclareRobustCommand{\PWpmu}{\HepParticle{\PW}{\mu}{+}\Xspace}
\DeclareRobustCommand{\PWmmu}{\HepParticle{\PW}{\mu}{-}\Xspace}
\DeclareRobustCommand{\PWpnu}{\HepParticle{\PW}{\nu}{+}\Xspace}
\DeclareRobustCommand{\PWmnu}{\HepParticle{\PW}{\nu}{-}\Xspace}
\DeclareRobustCommand{\PZmu}{\HepParticle{\PZ}{\mu}{}\Xspace}
\DeclareRobustCommand{\PZnu}{\HepParticle{\PZ}{\nu}{}\Xspace}
%--
\DeclareRobustCommand{\PXpm}{\HepParticle{\PX}{}{\pm}\Xspace}
\DeclareRobustCommand{\PXp}{\HepParticle{\PX}{}{+}\Xspace}
\DeclareRobustCommand{\PXm}{\HepParticle{\PX}{}{-}\Xspace}
\DeclareRobustCommand{\PYz}{\HepParticle{\PY}{Z}{}\Xspace}
\DeclareRobustCommand{\PYa}{\HepParticle{\PY}{A}{}\Xspace}
%
%\DeclareRobustCommand{\PAXpm}{\HepParticle{\mybar{\PX}}{}{pm}\Xspace}
%\DeclareRobustCommand{\PAXp}{\HepParticle{\mybar{\PX}}{}{+}\Xspace}
%\DeclareRobustCommand{\PAXm}{\HepParticle{\mybar{\PX}}{}{-}\Xspace}
%\DeclareRobustCommand{\PAYz}{\HepParticle{\mybar{\PY}}{Z}{}\Xspace}
%\DeclareRobustCommand{\PAYa}{\HepParticle{\mybar{\PY}}{A}{}\Xspace}
%
\DeclareRobustCommand{\PAXpm}{\HepAntiParticle{\PX}{}{\,\pm}\Xspace}
\DeclareRobustCommand{\PAXp}{\HepAntiParticle{\PX}{}{\,+}\Xspace}
\DeclareRobustCommand{\PAXm}{\HepAntiParticle{\PX}{}{\,-}\Xspace}
\DeclareRobustCommand{\PAYz}{\HepAntiParticle{\PY}{\,\PZ}{}\Xspace}
\DeclareRobustCommand{\PAYa}{\HepAntiParticle{\PY}{\,\PA}{}\Xspace}
%
\newcommand{\POZ}{{\overline{\PZ}}}
\newcommand{\POA}{{\overline{\PA}}}
\newcommand{\POH}{{\overline{\PH}}}
\newcommand{\POp}{{\overline{\upphi}}}
%--
%\DeclareRobustCommand{\POppm}{\HepParticle{\mybar{\upphi}}{}{\pm}\Xspace}
%\DeclareRobustCommand{\POpp}{\HepParticle{\mybar{\upphi}}{}{+}\Xspace}
%\DeclareRobustCommand{\POpm}{\HepParticle{\mybar{\upphi}}{}{-}\Xspace}
%\DeclareRobustCommand{\POpz}{\HepParticle{\mybar{\upphi}}{}{0}\Xspace}
%
\DeclareRobustCommand{\POppm}{\HepAntiParticle{\upphi}{}{\,\pm}\Xspace}
\DeclareRobustCommand{\POpp}{\HepAntiParticle{\upphi}{}{\,+}\Xspace}
\DeclareRobustCommand{\POpm}{\HepAntiParticle{\upphi}{}{\,-}\Xspace}
\DeclareRobustCommand{\POpz}{\HepAntiParticle{\upphi}{}{\,0}\Xspace}
%--
\DeclareRobustCommand{\Ppp}{\HepParticle{\upphi}{}{+}\Xspace}
\DeclareRobustCommand{\Ppm}{\HepParticle{\upphi}{}{-}\Xspace}
\DeclareRobustCommand{\Ppz}{\HepParticle{\upphi}{}{0}\Xspace}
%
\DeclareRobustCommand{\PpsiL}{\HepParticle{\uppsi}{L}{}\Xspace}
\DeclareRobustCommand{\PpsiR}{\HepParticle{\uppsi}{R}{}\Xspace}
\DeclareRobustCommand{\POpsiL}{\HepParticle{\mybar{\uppsi}}{L}{}\Xspace}
\DeclareRobustCommand{\POpsiR}{\HepParticle{\mybar{\uppsi}}{R}{}\Xspace}
\DeclareRobustCommand{\PQtR}{\HepParticle{\PQt}{R}{}\Xspace}
\DeclareRobustCommand{\PQbR}{\HepParticle{\PQb}{R}{}\Xspace}
%-
\newcommand{\pdmu}{{\partial_{\mu}}}
\newcommand{\pdnu}{{\partial_{\nu}}}
%
\newcommand{\myGF}{G_{\ssF}}
\DeclareRobustCommand{\PK}{\HepParticle{K}{}{}\Xspace}
\DeclareRobustCommand{\PKdag}{\HepParticle{\PK}{}{\dagger}\Xspace}
\newcommand{\KdK}{\lpar \PKdag\,\PK\rpar }
%
\DeclareRobustCommand{\Pxi}{\HepParticle{\upxi}{}{}\Xspace}
\DeclareRobustCommand{\Pxip}{\HepParticle{\upxi}{}{+}\Xspace}
\DeclareRobustCommand{\Pxim}{\HepParticle{\upxi}{}{-}\Xspace}
\DeclareRobustCommand{\Pxiz}{\HepParticle{\upxi}{}{0}\Xspace}
\DeclareRobustCommand{\Pxid}{\HepParticle{\upxi}{}{\dagger}\Xspace}
%
\newcommand{\dPK}{{\partial\PK}}
\newcommand{\essV}{{\mathrm{e}\PV}}
%\DeclareRobustCommand{\PAf}{\HepParticle{\mybar{\Pf}}{}{}\Xspace}
\DeclareRobustCommand{\PAf}{\HepAntiParticle{\Pf}{}{}\Xspace}
\newcommand{\Lag}{{\cal L}}
\newcommand{\Ope}{{\cal O}}
\newcommand{\Amp}{{\cal M}}
%
\DeclareRobustCommand{\xiW}{\HepParticle{\upxi}{\PW}{}\Xspace}
\DeclareRobustCommand{\xiZ}{\HepParticle{\upxi}{\PZ}{}\Xspace}
\DeclareRobustCommand{\OxiZ}{\HepParticle{\mybar{\upxi}}{\PZ}{}\Xspace}
\DeclareRobustCommand{\OxiZs}{\HepParticle{\mybar{\upxi}}{\PZ}{2}\Xspace}
%
\DeclareRobustCommand{\PWpL}{\HepParticle{\PW}{\PL}{+}\Xspace}
\DeclareRobustCommand{\PWmL}{\HepParticle{\PW}{\PL}{-}\Xspace}
%
\newcommand{\Fsc}{\mu^2_{\ssF}}
\newcommand{\Rsc}{\mu^2_{\ssR}}
%
\DeclareRobustCommand{\Ph}{\HepParticle{h}{}{}\Xspace}
\DeclareRobustCommand{\PHpm}{\HepParticle{\PH}{}{\pm}\Xspace}
\DeclareRobustCommand{\PHp}{\HepParticle{\PH}{}{+}\Xspace}
\DeclareRobustCommand{\PHm}{\HepParticle{\PH}{}{-}\Xspace}
\DeclareRobustCommand{\Pft}{\HepParticle{\tilde{\Pf}}{}{}\Xspace}
\DeclareRobustCommand{\Pcpmi}{\HepParticle{\upchi}{i}{\pm}\Xspace}
\DeclareRobustCommand{\Pcpi}{\HepParticle{\upchi}{i}{+}\Xspace}
\DeclareRobustCommand{\Pcmi}{\HepParticle{\upchi}{i}{-}\Xspace}
\DeclareRobustCommand{\Pci}{\HepParticle{\upchi}{i}{}\Xspace}
%
\newcommand{\srt}{\sqrt{2}}
\newcommand{\PWW}{\PW\PW}
\newcommand{\PZZ}{\PZ\PZ}
%
\DeclareRobustCommand{\PdT}{\HepParticle{\mytil{\PF}}{\mu\nu}{a}\Xspace}
\DeclareRobustCommand{\HB}{\HepAntiParticle{\PH}{}{}\Xspace}
\DeclareRobustCommand{\PZB}{\HepAntiParticle{\PZ}{}{}\Xspace}
\DeclareRobustCommand{\myPAB}{\HepAntiParticle{\PA}{}{}\Xspace}
\DeclareRobustCommand{\OM}{\HepAntiParticle{\PM}{}{}\Xspace}
\DeclareRobustCommand{\OMs}{\HepAntiParticle{\PM}{}{\,2}\Xspace}
\DeclareRobustCommand{\OMzs}{\HepAntiParticle{\PM}{\,0}{\,2}\Xspace}
\DeclareRobustCommand{\OMzq}{\HepAntiParticle{\PM}{\,0}{\,4}\Xspace}
\DeclareRobustCommand{\OMH}{\HepAntiParticle{\PM}{\,\PH}{}\Xspace}
\DeclareRobustCommand{\OMHs}{\HepAntiParticle{\PM}{\,\PH}{\,2}\Xspace}
\DeclareRobustCommand{\OMHq}{\HepAntiParticle{\PM}{\,\PH}{\,4}\Xspace}
\DeclareRobustCommand{\phib}{\HepAntiParticle{\upphi}{}{}\Xspace}
\newcommand{\ACf}{\frac{\OMs}{\HSs}}
%
\DeclareRobustCommand{\PHb}{\HepParticle{\mathbf{H}}{}{}\Xspace}
\DeclareRobustCommand{\PAb}{\HepParticle{\mathbf{A}}{}{}\Xspace}
\DeclareRobustCommand{\PZb}{\HepParticle{\mathbf{Z}}{}{}\Xspace}
\DeclareRobustCommand{\PWb}{\HepParticle{\mathbf{W}}{}{}\Xspace}
\DeclareRobustCommand{\PWpb}{\HepParticle{\mathbf{W}}{}{+}\Xspace}
\DeclareRobustCommand{\PWmb}{\HepParticle{\mathbf{W}}{}{-}\Xspace}
\DeclareRobustCommand{\Pgb}{\HepParticle{\mathbf{g}}{}{}\Xspace}
\DeclareRobustCommand{\PGgb}{\HepParticle{\mathbf{\mathbf{\upgamma}}}{}{}\Xspace}
\DeclareRobustCommand{\PQtb}{\HepParticle{\mathbf{t}}{}{}\Xspace}
\DeclareRobustCommand{\PAQtb}{\HepAntiParticle{\mathbf{t}}{}{}\Xspace}
\DeclareRobustCommand{\PQbb}{\HepParticle{\mathbf{b}}{}{}\Xspace}
\DeclareRobustCommand{\PAQbb}{\HepAntiParticle{\mathbf{b}}{}{}\Xspace}
\DeclareRobustCommand{\Pfb}{\HepParticle{\mathbf{f}}{}{}\Xspace}
\DeclareRobustCommand{\PAfb}{\HepAntiParticle{\mathbf{f}}{}{}\Xspace}
%
\newcommand{\ugm}{\upgamma}
\newcommand{\ougm}{{\overline{\upgamma}}}
\newcommand{\cent}{\mathrm{c}}
%
\providecommand\Table{Table}
\providecommand*\Tref[1]{\Table~\ref{#1}}
%
\providecommand\Section{Section}
\providecommand*\Sref[1]{\Section~\ref{#1}}
%

